Finding an $\epsilon$-close Variation of Parameters in Bayesian Networks

This paper addresses the $\epsilon$-close parameter tuning problem for Bayesian Networks (BNs): find a minimal $\epsilon$-close amendment of probability entries in a given set of (rows in) conditional probability tables that make a given quantitative constraint on the BN valid. Based on the state-of-the-art "region verification" techniques for parametric Markov chains, we propose an algorithm whose capabilities go beyond any existing techniques. Our experiments show that $\epsilon$-close tuning of large BN benchmarks with up to 8 parameters is feasible. In particular, by allowing (i) varied parameters in multiple CPTs and (ii) inter-CPT parameter dependencies, we treat subclasses of parametric BNs that have received scant attention so far.

==> discussion.tex <==
\begin{comment}
\section{Discussion, Related, and Future Work }
Our parameter tuning approach is inherently not restricted to a specific distance measure or to a specific parametrization scheme as it makes no assumption on the form of the pBN sensitivity function and how the network is parameterized. Most interestingly, by allowing inter-CPTs parameter dependencies, we address pBNs that may yield sensitivity functions that are not necessarily multi-linear in the varied parameters. Rather than explicitly computing the sensitivity functions that are hard to interpret and hard to analyze \cite{}, we take the pMC of the pBN and exploit the approximate methods to tune the parameters.
For our experimental evaluation, we opted for the proportional co-variation scheme that is most established in the literature and has several useful characteristics: it is valid, domain-independent, linear, point-wise linear, and it preserves the original values of the co-varied entries if a parameter remains the same. Most importantly, as empirically indicated by \cite{}, it optimizes the CD-distance compared to other parametrization schemes for several pBN subclasses. Further research is needed to formally prove such optimization results and extend those results to other pBN subclasses. 
For the general case, we expect that (i) providing model-checking feedback from the previous iterations, (ii) providing the monotonicity information of the parameters, and (iii) implementing heuristics for picking the subregions are beneficial to accelerate the partitioning step. 
It is also interesting for future work to take pBN benchmarks from other parametrization schemes such as balanced tuning heuristics\cite{} and order-preserving \cite{} that in some special use-cases are useful, ex., When the probability values in the CPTs in the original networks have a specific order imposed by the domain.  \textcolor{blue}{to revize}
\end{comment}

==> plots/coverage-plots-side-by-side.tex <==
 \begin{figure*}[btp]
     \centering
       \begin{minipage}{0.005\linewidth}
  \end{minipage}
  \hfill
   \subfloat[]{
   \centering
     \begin{minipage}{0.32\linewidth}
     \centering
      \resizebox{1.0\width }{0.85\height}{%
       \input{plots/coverage-time.tex}
	}
	\end{minipage}
   }
   \hfill
   \centering
  \subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
      \resizebox{1.0\width }{0.85\height}{%
  \input{plots/coverage-bayesdiff.tex}
	}
	\end{minipage}
		%
	}
	\hfill
	\centering
\subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
  \resizebox{1.0\width }{0.85\height}{%
  \input{plots/coverage-iteration.tex}
  }
  \end{minipage}
  }
  \hfill
  \begin{minipage}{0.005\linewidth}
  
  \end{minipage}
     \caption{\textcolor{blue}{add caption}.}
     \label{fig:coverage-experiments}
 \end{figure*}

==> plots/storm-bayesserver-plots-side-by-side.tex <==
 \begin{figure*}[btp]
     \centering
       \begin{minipage}{0.005\linewidth}
  \end{minipage}
  \hfill
   \subfloat[]{
   \centering
     \begin{minipage}{0.32\linewidth}
     \centering
      \resizebox{0.6\width }{0.6\height}{%
       \input{plots/iteration-storm-baysserver.tex}
	}
	\end{minipage}
   }
   \hfill
   \centering
  \subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
      \resizebox{1.0\width }{0.9\height}{%
  \input{plots/storm-vs-bayesserver-time.tex}
	}
	\end{minipage}
		%
	}
	\hfill
	\centering
\subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
  \resizebox{1.0\width }{0.9\height}{%
  \input{plots/coverage-bayesdiff.tex}
  }
  \end{minipage}
  }
  \hfill
  \begin{minipage}{0.005\linewidth}
  
  \end{minipage}
     \caption{\textcolor{blue}{add caption}.}
     \label{fig:tuning-experiments-plots-coverage-bayesserver}
 \end{figure*}

==> plots/tuning-plots-side-by-side.tex <==
 \begin{figure*}[!h]
     \centering
      \resizebox{0.8\width }{0.8\height}{
       \begin{minipage}{0.005\linewidth}
  \end{minipage}
  \hfill
   \subfloat[]{
   \centering
     \begin{minipage}{0.32\linewidth}
     \centering
      \resizebox{1.0\width }{0.95\height}{%
       \input{plots/time-threshhold.tex}
	}
	\end{minipage}
   }
   \hfill
   \centering
  \subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
      \resizebox{1.0\width }{0.95\height}{%
  \input{plots/distance-threshhold.tex}
	}
	\end{minipage}
		%
	}
	\hfill
	\centering
\subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
  \resizebox{1.0\width }{0.95\height}{%
  \input{plots/iteration-threshhold.tex}
  }
  \end{minipage}
  }
 
  
  \hfill
  \begin{minipage}{0.005\linewidth}
  
  \end{minipage}
  }
  
   \resizebox{0.8\width }{0.8\height}{
  \begin{minipage}{0.005\linewidth}
  \end{minipage}
  \hfill
   \subfloat[]{
   \centering
     \begin{minipage}{0.32\linewidth}
     \centering
      \resizebox{1.0\width }{0.95\height}{%
       \input{plots/coverage-samiamdiff.tex}
	}
	\end{minipage}
   }
   \hfill
   \centering
  \subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
      \resizebox{1.0\width }{0.95\height}{%
  \input{plots/coverage-bayesdiff.tex}
	}
	\end{minipage}
		%
	}
	\hfill
	\centering
\subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
  \resizebox{1.0\width }{0.95\height}{%
  \input{plots/coverage-iteration.tex}
  }
  \end{minipage}
  }
  \hfill
  \begin{minipage}{0.005\linewidth}
  \end{minipage}
  }

   \resizebox{0.8\width }{0.8\height}{
         \begin{minipage}{0.005\linewidth}
  \end{minipage}
   \hfill
   \centering
  \subfloat[
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
      \resizebox{1.0\width }{0.9\height}{%
  \input{plots/coverage-time.tex}
	}
	\end{minipage}
		%
	}
	\hfill
	\centering
\subfloat[ \textcolor{blue}{A few more benchmarks are to be added to this plot}
  ]{ 
  \centering
  \begin{minipage}{0.32\linewidth}
  \centering
  \resizebox{1.0\width }{0.9\height}{%
  \input{plots/storm-vs-bayesserver-time.tex}
  }
  \end{minipage}
  }
    \hfill
   \subfloat[\textcolor{blue}{}]{
   \centering
     \begin{minipage}{0.32\linewidth}
     \centering
      \resizebox{0.6\width }{0.6\height}{%
       \input{plots/iteration-storm-baysserver.tex}
	}
	\end{minipage}
   }
  \hfill
  \begin{minipage}{0.005\linewidth}
  \end{minipage}
  }
  
     \caption{The sensitivity of region-based minimal-change parameter tuning on the constraint's threshold, refinement factor, and the region expansion factor; the experimental results for $p_1c_1r_1$ subclass.}
     
     \label{fig:threshhold-tuning-experiments}
 \end{figure*}


==> pseudocodes/minimal-tuning-pseudocode.tex <==
\newcommand{\Cross}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.2ex] \draw (0,0) -- (1,1) (0,1) -- (1,0);}}%

\begin{algorithm}[!h]
   % \KwIn{pMC $\mathcal{M_{\B}}=(S,s_I,X,P)$, the initial instantiation $u_0$, the specification $\varphi$, the coverage factor $\eta$, and the configuration $(\gamma, K)$ }
   % \vspace{0.5cm}
   
    
   $\M_{\B} \leftarrow \computeMC(\B)$ \tcp*{See Section \ref{subsec:pBN2pMC}}
   
   $\varrho\leftarrow \reachSpec(\phi)$ \tcp*{See Section \ref{subsec:pBN2pMC}}
   
    $\epsilon_0 \leftarrow \sqrt{n} \cdot \gamma^{K{-}1}$
    
     $\epsilon \leftarrow \epsilon_0$ 
     

     \Fn{\tuning{$\M_{\B},u_0,\varphi,\eta$}}{
     
    \While{$\epsilon \leq \sqrt{n}$}{
    
    $R_+ \leftarrow\, $\FEpPartition{$\mathcal{M_{\B}},\varphi,\epsilon,\eta$}
    
    \tcp{No accepting subregion}
    
    \eIf{$R_+ = \emptyset$}{
    
     $\epsilon \leftarrow  \gamma^{-1} \cdot \epsilon$
    
    }{ 
    
    \tcp{See Algorithm \ref{alg:minimal-inst}}%, subsection \ref{method:subsec2}.}
    
       \KwRet{$\FminimalInst(R_{+},u_0)$}
    
    }
    }
    
    \KwRet{\NotFeas}
    }
    
   \vspace{0.5cm}
   
     \Fn{\FEpPartition{$\mathcal{M_{\B}},\varphi,\epsilon,\eta$}}{
  
  \tcp{Build region $R_{\epsilon}$}

  $R_{\epsilon} \leftarrow \Cross_{x_j \in X} \, [u_0(x_j) {-} \frac{\epsilon}{\sqrt{n}}, u_0(x_j) {+} \frac{\epsilon}{\sqrt{n}}]$
   % $R_{\epsilon} \leftarrow x_j \in [u_0(x_j) - \frac{\epsilon}{\sqrt{n}}, u_0(x_j) + \frac{\epsilon}{\sqrt{n}}]$ for  each $x_j \in X$
    
      \tcp{See Section \ref{subsec:pla}}

         {$R_{+}, R_{-}, R_{?} \leftarrow \PSP(\mathcal{M_{\B}}, R_{\epsilon}, \varphi, \eta)$}
         
{ \KwRet{$R_+$}
}
}
\caption{Minimal change parameter tuning}
\label{alg:minimal-change}
\end{algorithm}

==> pseudocodes/minimal-tuning-revised.tex <==
\newcommand{\Cross}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.2ex] \draw (0,0) -- (1,1) (0,1) -- (1,0);}}%

\begin{algorithm}[!h]
\scriptsize
   % \KwIn{pMC $\mathcal{M_{\B}}=(S,s_I,X,P)$, the initial instantiation $u_0$, the specification $\varphi$, the coverage factor $\eta$, and the configuration $(\gamma, K)$ }
   % \vspace{0.5cm}
   
    
   $\M_{\B} \leftarrow \computeMC(\B)$
   
   $\varrho\leftarrow \reachSpec(\phi)$
   
    $\epsilon_0 \leftarrow \hat{d_0} \cdot \gamma^{K{-}1}$
    
     $\epsilon \leftarrow \epsilon_0$ 
     

     \Fn{\tuning{$\M_{\B},u_0,\varphi,\eta$}}{
     
    \While{$\epsilon \leq \hat{d_0}$}{
    
    $R_+ \leftarrow\, $\FEpPartition{$\mathcal{M_{\B}},\varphi,\epsilon,\eta$}
        
    \eIf{$R_+ = \emptyset$}{
    
     $\epsilon \leftarrow  \gamma^{-1} \cdot \epsilon$
    
    }{ 
        
       \KwRet{$\FminimalInst(R_{+},u_0)$}
    
    }
    }
    
    \KwRet{\NotFeas}
    }
    
   \vspace{0.15cm}
   
     \Fn{\FEpPartition{$\mathcal{M_{\B}},\varphi,\epsilon,\eta$}}{
  
  $R_{\epsilon} \leftarrow \Cross_{x_j \in X} \, [u_0(x_j) {-} \frac{\epsilon}{n}, u_0(x_j) {+} \frac{\epsilon}{n}]$
   % $R_{\epsilon} \leftarrow x_j \in [u_0(x_j) - \frac{\epsilon}{\sqrt{n}}, u_0(x_j) + \frac{\epsilon}{\sqrt{n}}]$ for  each $x_j \in X$
    
         {$R_{+}, R_{-}, R_{?} \leftarrow \PSP(\mathcal{M_{\B}}, R_{\epsilon}, \varphi, \eta)$}
         
{ \KwRet{$R_+$}
}
}
\caption{Minimal change tuning}
\label{alg:minimal-change}
\end{algorithm}


==> pseudocodes/region-expansion-pseudocode.tex <==
\begin{algorithm}[!ht]
\scriptsize
\Fn{\expandRegionEC{$u_0,\epsilon$}}{
  $R_{\epsilon} \leftarrow \Cross_{x_j \in X} \, [u_0(x_j) {-} \frac{\epsilon}{n}, u_0(x_j) {+} \frac{\epsilon}{n}]$ \\
   % $R_{\epsilon} \leftarrow x_j \in [u_0(x_j) - \frac{\epsilon}{\sqrt{n}}, u_0(x_j) + \frac{\epsilon}{\sqrt{n}}]$ for  each $x_j \in X$
   \KwRet{$R_{\epsilon}$}
}

   \vspace{0.15cm}

\Fn{\expandRegionCD{$u_0,\epsilon$}}{
$\alpha \leftarrow e^{\nicefrac{\epsilon}{2}}$ \\
  $R_{\epsilon} \leftarrow \Cross_{x_j \in X} \, [u_0(x_j) \cdot \alpha^{-1}, u_0(x_j) \cdot \alpha]$ \\
   % $R_{\epsilon} \leftarrow x_j \in [u_0(x_j) - \frac{\epsilon}{\sqrt{n}}, u_0(x_j) + \frac{\epsilon}{\sqrt{n}}]$ for  each $x_j \in X$
   \KwRet{$R_{\epsilon}$}
}
\caption{$\epsilon$-close sub-regions}
\label{alg:epsilon-close}
\end{algorithm}



==> tables/alarm-multiple-par.tex <==

%%%%%%%%% alarm
%\begin{table*}[!btp]
%	\centering
	\scalebox{0.80}{
			\begin{tabular}{ccrrrrr}
			%		\label{tab:mutiple-par-alarm}
		\toprule
		\multicolumn{2}{c}{pBN info} & \multicolumn{1}{c}{constraint} & setting & \multicolumn{3}{c}{results} \\ 
		 \cmidrule(lr){1-2} \cmidrule(lr){3-3}
\cmidrule(lr){4-4} \cmidrule(lr){5-7} 
 pCPT   & par. & thresh. & cover. & EC & iter & \textbf{t}(s)  \\ \midrule
%	\texttt{alarm}           & $p_1c_1r_1$       & 1  & $\leq 0.40$ & 1118 & 3174  & 99.99\%    &  0, Sat & 1 & 0 & 1.978 &  ns & ns & ns & ns & ns\\
	%	\texttt{alarm}  & $p_1c_1r_1$       & 1  & $\leq 0.39$ & 1118 & 3174  & 99.99\%    &  0.000875 & x & 1 & 1.957 &  ns & ns & ns & ns & ns\\
		 $1$       & 2  & $\leq 0.30$  & 70\%    &   Not found & 6 & 2.073 \\
	 $1$       & 2  & $\leq 0.30$   & 85\%    &  1.138343094  & 5 & 2.090 \\
$1$       & 2  & $\leq 0.30$  & 99\%    &  1.091371208   & 5 & 2.134 \\
 $1$       & 2  & $\leq 0.30$  & 99.99\%    &  1.090202067    & 5 & 302.1 \\
	$1$       & 2  & $\leq 0.25$ & 100\%    &  Infeasible  & 6 & 1.862 \\
		%\texttt{alarm}           & $p_4c_1r_4$       & 4  & $\leq 0.30$ & 1118 & 3174  & 50\%    & 1.024841451 & x & 5 & 1.862  &  ns & ns & ns & ns & ns\\
 $1$       & 4  & $\leq 0.30$   & 70\%    & 0.909491616 &  5 & 5.701 \\
	 $1$       & 4  & $\leq 0.30$   & 85\%    & 0.890217670 & 5 & 142.1 \\
$1$       & 4  & $\leq 0.30$   & 90\%    & - & -  & TO\\
	$1$       & 4  & $\leq 0.20$  & 100\%    & Infeasible &  6 & 1.869 \\
			 $1$       & 8  & $\leq 0.30$ & 20\%    & 0.5628159113 & 5 & 534.6  \\
		$1$       & 8  & $\leq 0.25$  & 20\%    & 0.9405485102 & 5 & 216.6 \\
	 $1$       & 8  & $\leq 0.20$ & 20\%    & 1.010395962 &  6 & 305.9\\
$1$       & 8  & $\leq 0.001$ & 100\%    & Infeasible  & 6 & 1.886  \\
	        \bottomrule
			\end{tabular}
	}
%\caption{The scalability of our approach to pBNs with multiple parameters, detailed results for \texttt{alarm} network.}
%\end{table*}


==> tables/side-by-side-table-par.tex <==

\begin{table*}[!b]
\begin{tabular}{ll}
\input{tables/win95pts-multiple-par-dep.tex}
&
\input{tables/alarm-multiple-par-dep.tex}
\end{tabular}
\caption{The scalability of our approach to pBNs with multiple parameters, detailed results for (left) \texttt{win95pts} and (right) \texttt{alarm}. The parametric distributions (pDistr) marked with $*$ indicate parameter dependencies.}
\label{tab:multi-par-results}
\end{table*}

==> tables/win95pts-multiple-par.tex <==
%\begin{table*}[!h]
	%\centering
		\scalebox{0.80}{
			\begin{tabular}{ccrrrrr}
				%	\label{tab:mutiple-par-win95pts}
		\toprule
		\multicolumn{2}{c}{pBN info} & \multicolumn{1}{c}{constraint} & setting & \multicolumn{3}{c}{results} \\ 
		 \cmidrule(lr){1-2} \cmidrule(lr){3-3}
\cmidrule(lr){4-4} \cmidrule(lr){5-7} 
 pCPT   & par. & thresh. & cover. & EC & iter & \textbf{t}(s)  \\ \midrule
%	\texttt{win95pts}           & $p_1c_1r_1$       & 1  & x & 9,947 & 17,948  & x   &  x & x & x & x &  ns & ns & ns & ns & ns\\
	%	\texttt{win95pts}  & $p_1c_1r_1$        & 1  & x & 9,947 & 17,948  & x   &  x & x & x & x &  ns & ns & ns & ns & ns\\
		%	\texttt{win95pts}           & $p_2c_1r_1$       & 2  & $\leq 0.113$ & 9,947 & 17,948  & 99\%   &  0.4077036493& x & 4 &  4.503 &  ns & ns & ns & ns & ns\\
	%\texttt{win95pts}           & $p_2c_1r_2$       & 2  & $\leq 0.113$ & 9,947 & 17,948  & 99.99\%   &  0.4074670004 & x & 4 & 625.5 &  ns & ns & ns & ns & ns\\
		         $1$       & 2  & $\geq 0.115$ & 99\%   &  0.8365285878 & 5 & 4.200 \\
			%          $p_2c_1r_2$       & 2  & $\geq 0.115$& 99.99\%   &  0.8355019545 & 5 & 587.7 \\
				 $1$       & 2  & $\geq 0.25$  & 100\%   &  Infeasible &6 & 3.750 \\
				 $3$       & 4  & $\geq 0.115$  & 90\%   &  0.1350477346 & 2 & 5.210 \\
		   		 $3$       & 4  & $\geq 0.25$  & 80\%   &  0.4479118217 & 4 & 5.210 \\
				 $3$       & 4  & $\geq 0.25$  & 90\%   &  0.4238956239 & 4 & 30.82 \\
		        $3$       & 4 & $\geq 0.25$  & 95\%   &  0.4098399078 & 4 & 1128.5 \\
			     $3$       & 4 & $\geq 0.25$ &  99\%   &  - & - & TO \\
				 $4$       & 8  & $\geq 0.115$  & 80\%   &  0.8805679985 & 2 & 4.496 \\
			     $4$       & 8  & $\geq 0.115$  & 90\%   &  0.1350477346 & 2 & 15.91\\
			     $4$       & 8  & $\geq 0.25$  & 60\%   &  0.8094516663 &  5 &  206.1 \\			
		        $4$       & 8  & $\geq 0.30$ & 60\%   &  0.8805679985 & 6 & 809.7 \\
				   $4$       & 8  & $\geq 0.35$  & 99.99\%   &  Infeasible & 6 & 3.757 \\
			        $4$       & 16 & $\geq 0.35$  & 10\%   &  - & 1 & MO \\
	        \bottomrule
			\end{tabular}
	}
%\caption{The pBNs with multiple parameters, detailed results for \texttt{win95pts}. }
%\end{table*}

